Kinematically-Decoupled Impedance Control for Fast Object Visual Servoing and Grasping on Quadruped Manipulators

We propose a control pipeline for SAG (Searching, Approaching, and Grasping) of objects, based on a decoupled arm kinematic chain and impedance control, which integrates image-based visual servoing (IBVS). The kinematic decoupling allows for fast end-effector motions and recovery that leads to robust visual servoing. The whole approach and pipeline can be generalized for any mobile platform (wheeled or tracked vehicles), but is most suitable for dynamically moving quadruped manipulators thanks to their reactivity against disturbances. The compliance of the impedance controller makes the robot safer for interactions with humans and the environment. We demonstrate the performance and robustness of the proposed approach with various experiments on our 140 kg HyQReal quadruped robot equipped with a 7-DoF manipulator arm. The experiments consider dynamic locomotion, tracking under external disturbances, and fast motions of the target object.

==> 07_bibliography.tex <==
\begin{thebibliography}{99}
 \bibitem{WBC ALMA} C. Dario Bellicoso, K Kramer, Markus Stäuble, Dhionis Sako, Fabian Jenelten, Marco Bjelonic, Marco Hutter. \textit{ALMA - Articulated Locomotion and Manipulation for a Torque-Controllable Robot}.

\bibitem[MPC ALMA]{}
J. -P. Sleiman, F. Farshidian, M. V. Minniti and M. Hutter, "A Unified MPC Framework for Whole-Body Dynamic Locomotion and Manipulation," in IEEE Robotics and Automation Letters, vol. 6, no. 3, pp. 4688-4695, July 2021, doi: 10.1109/LRA.2021.3068908.

%Xin, G., Wolfslag, W.J., Lin, H., Tiseo, C., Mistry, M.N. (2020). An Optimization-Based Locomotion Controller for Quadruped Robots Leveraging Cartesian Impedance Control. Frontiers in Robotics and AI, 7.
\end{thebibliography}


